Mini-BEHAVIOR: A Procedurally Generated Benchmark for Long-horizon Decision-Making in Embodied AI

We present Mini-BEHAVIOR, a novel benchmark for embodied AI that challenges agents to use reasoning and decision-making skills to solve complex activities that resemble everyday human challenges. The Mini-BEHAVIOR environment is a fast, realistic Gridworld environment that offers the benefits of rapid prototyping and ease of use while preserving a symbolic level of physical realism and complexity found in complex embodied AI benchmarks. We introduce key features such as procedural generation, to enable the creation of countless task variations and support open-ended learning. Mini-BEHAVIOR provides implementations of various household tasks from the original BEHAVIOR benchmark, along with starter code for data collection and reinforcement learning agent training. In essence, Mini-BEHAVIOR offers a fast, open-ended benchmark for evaluating decision-making and planning solutions in embodied AI. It serves as a user-friendly entry point for research and facilitates the evaluation and development of solutions, simplifying their assessment and development while advancing the field of embodied AI. Code is publicly available at https://github.com/StanfordVL/mini_behavior.

==> old.tex <==
% \section{Mini-BEHAVIOR}
% The Mini-BEHAVIOR environment is built on top of the MiniGrid library, so it inherits aspects such as the basic design and simplicity of the Gridworld environment \cite{MinigridMiniworld23}. 

% However, MiniGrid is only able to support a small range of goal-oriented tasks because of its limited action space for interacting with the environment and physical grid constraints. In particular, each cell is only allowed to have one object, and that each object takes up exactly one cell. The implication of these constraints is that MiniGrid only has 2 dimensions, and there are no notions of size, height, and vertical or internal placement. For example, both an apple and a bed have the same effective size and height, and it is not possible to place a pan on top of a counter or an apple inside the refrigerator.

% With Mini-BEHAVIOR, we extend MiniGrid's capabilities and add key features such as a third vertical dimension, multi-cell objects, support for symbolic states, and unlimited tasks, actions, and objects. These features are critical to support implementations of realistic, long-horizon BEHAVIOR tasks in a Gridworld environment.

% In this section, we discuss the Mini-BEHAVIOR environment, agent, and features of the benchmark to support the development of planning algorithms, including symbolic and visual approaches.

% \subsection{Environment}

% In Mini-BEHAVIOR, each environment is represented as a rectangular grid of $n \times m$ cells, with each cell containing 3 vertical dimensions (top, middle, bottom). Each dimension can contain up to one object. While this is not entirely reflective of the real world, 3 dimensions are enough to support all of the BEHAVIOR tasks and most real-world scenarios.

% By default, the layout of the environment is a $20\times20$ grid with walls along the outside. However, the layout is easily customizable by changing the grid size and/or adding additional \textit{Room} and \textit{Wall} objects to the grid. There are parameters which can be used to set the size and create grids of rooms, and we also provide some default layouts that correspond to scene layouts from iGibson (Figure \ref{fig:env_layouts}). If more customization is needed, it is also easy to manually add walls to the environment class.

% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{env_layouts.png}
%     \caption{Examples of Mini-BEHAVIOR environment layouts: one $20\times20$ room (left), four $6\times6$ rooms (middle), iGibson \texttt{Rs\_int} scene layout (right)}
%     \label{fig:env_layouts}
% \end{figure}

% \subsection{Objects}
% We define two classes of objects: an object class and a furniture class. 

% \textit{Objects} are objects that we often move or pick up in our everyday lives, such as a book, apple, or towel. On the other hand, \textit{furniture} objects remain stationary and include common household furniture such as a table, bed, refrigerator, and stove. In the real world, furniture is generally larger in both size and height, and Mini-BEHAVIOR supports this distinction. \textit{Objects} are defined to be $1\times1\times1$ in size, while furniture can span multiple cells and vertical dimensions.

% Following iGibson, we define abilities for each object, where these abilities represent the kinds of actions that can be performed on them. For example, all \textit{objects} have the abilities of \textit{pickup-able} and \textit{place-able}, but some objects like a towel, apple, and butter have additional abilities of being \textit{soak-able}, \textit{slice-able},  and \textit{freeze-able}. On the other hand, \textit{furniture} like a \textit{stovetop} is \textit{toggle-able} and a refrigerator is \textit{open-able}.



% \subsection{Symbolic States}
% We define 3 types of states: agent-related, absolute, and relative object states. Agent-related and absolute object states are unary, while relative object states are binary.  A complete list of the provided states are in the following table:

% \begin{center}
% \begin{tabular}{ |c|c|c| } 
%  \hline
%  State & Type & Description \\ 
%  \hline 
%  InFOV & agent & object is in the cell in front of the agent \\
%   \hline
%  InHand & agent & object is in the hand of the agent \\ 
%  \hline
%  InReach & agent & object is either in front or in hand of agent \\ 
%  \hline
%  InSameRoom & agent & object is in the same room as the agent \\ 
%  \hline
%  Cooked & absolute & the object is cooked (only food objects) \\
%   \hline
%  Dusty & absolute & the object is dusty \\ 
%  \hline
%  Frozen & absolute & the object is frozen (only food objects)  \\ 
%  \hline
%  Opened & absolute & the object is open (refregirator, box, etc) \\ 
%  \hline
%  Sliced & absolute & the object is sliced (only food objects)  \\ 
%  \hline
%  Soaked & absolute & the object is soaked \\  
%  \hline
%  Stained & absolute & the object is stained \\
%  \hline
%  ToggledOn & absolute & the object is on \\  
%  \hline
%  OnFloor & absolute & object is on the floor \\ 
%  \hline 
%  AtSameLocation & relative & object1 and object2 are in the same cell \\ 
%  \hline
%  Inside & relative & object1 is inside object2 \\ 
%  \hline
%  NextTo & relative & object1 and object2 are in adjacent cells \\ 
%  \hline 
%  OnTop & relative & object1 is one dimension above object2 \\ 
%  \hline
%  Under & relative & object1 is one dimension below object2 \\ 
%  \hline
% \end{tabular}
% \end{center}  


% \subsection{Agent}

% \subsubsection{Action Space}
% By default, Mini-BEHAVIOR agent uses an action space that consists of primitive actions, resulting in a 15-dimensional discrete action space including 3 for navigation (forward, turn left, turn right) and 12
% for interacting with objects (close, cook, drop (3d), drop-in, open, pickup (3d), slice, toggle). Under this setting, the same action space is shared across different tasks, allowing the study of transfer learning, multi-task learning, and meta-learning. 

% A drawback of the primitive action space is that the agent can only carry one object at a time to prevent action ambiguity, which may cause inefficiency.
% Therefore, Mini-BEHAVIOR supports an additional type of action space - the cartesian action space - which allows for the simultaneous carrying of multiple objects. The cartesian action space consists of the cartesian product between the primitive actions and available objects for a given task, with invalid actions (e.g. "slice a refrigerator") removed. Such an action space makes carrying and dropping multiple objects possible, and is often better suited for studying how to solve a single task. However, the cartesian action space for different tasks will be different, based on the available objects. For a task where each object $i$ has $n_i$ possible actions, the action dimension of the cartesian action space is equal to $4 + \sum_{i} n_i$. This ranges from 5 (for the simplest task of installing a printer) to 54 (for preparing a salad).

% \subsubsection{Observation Space}
% Mini-BEHAVIOR supports both fully observable and partially observable environments. In the partially observable case, the observation space of the agent is a $7 \times 7 \times 31$ ego-centric grid; when fully observable, the observation space is a $n \times n \times 31$ global grid, where $n$ is the size of the map. Each 31-dimension pixel encodes the states of the furniture and up to three objects that occupy a given cell on the map.

% \subsubsection{Reward}
% By default, Mini-BEHAVIOR uses sparse rewards for all tasks, where the agent receives 1 for successfully completing the task, and 0 otherwise.
% The user can easily implement dense rewards for each environment, and toggle it on / off during environment initialization, where we provide examples in the following two tasks: putting away dishes after cleaning, and washing pots and pans.


% \subsection{Procedural Generation}
% With Mini-BEHAVIOR, we provide the capability to use procedural generation for scene instantiations. This is achieved through random floor plan generation and furniture/object placement:

% \textbf{1. Floor Plan Generation.}
% The floor plan of the grid household world environment is determined by the layout and arrangement of rooms, walls, doors. Marple Mini Behavior allows random floor plan generation by first generate the surrounding walls of the grid, random generate split walls in the grid so the grid is divided into two to form two rooms, and choose a room to continue the split. In the end, the environment $E$ will have $E_{w_s}$ split walls and $E_r = E_{w_s} + 1$ rooms. Doors are generated on the split walls and the number of doors are $E_d = E_{w_s}$.

% \textbf{2. Furniture/Object Placement.} The number of Furnitures in each room and Objects on each furniture are either predefined in configuration files for procedural generation mentioned in Section \ref{sec:usage} or randomly sampled from a range of $1 \sim \mathrm{max}(2, room.width \times room.height / 12)$ and $1 \sim furniture.width * furniture.height$. The types of furnitures in each room are randomly sampled from a room-furniture mapping if not specified in the configuration file, which means we only generate furniture instances that are usually placed in the room to simulate real life. For example, we usually have \texttt{toilet} in \texttt{Bathroom}, \texttt{sofa} in \texttt{LivingRoom}, \texttt{refrigerator} in \texttt{Kitchen} and \texttt{bed} in \texttt{Bedroom}. The types of objects on each furniture are randomly sampled from the object list the simulator supported. The positions of the furnitures are randomly sampled in the room, and the objects on each furniture are randomly sampled from the area where the furniture occupies, if not specified in the configurations.

% \section{Simulation Visualizations and Usage}
% To support visual agents and manual control of the environment, we provide various ways to visualize the environment as a grid rendering of $n\times m$ cells. The agent is represented by a red triangle, and walls are represented by gray cells. To visualize a 3D environment in a 2D format, we provide 3 different views of the environment -- default view, dimension view, and furniture view.

% \subsection{State Visualization}
% Only unary states are visualized, which means that the possible states are cooked, dusty, frozen, opened, sliced, soaked, stained, and toggledon for \textit{objects} (8 total) and dusty, opened, stained, toggledon for \textit{furniture} (4 total). 

% To visualize the \textit{object} states, there are 8 squares to the right edge of the object cell to represent the 8 possible states. The square is green if the state is True and red otherwise. 

% For \textit{furniture} states, note that all furniture is constrained to be rectangular, so we use the 4 edges to visualize the states (left: dusty, top: opened, right: stained, bottom: toggledon). In particular, a green edge indicates that a state is True.

% \subsection{Scene Visualization: Default View}
% We provide three ways to view the grid, each with their own characteristics and trade-offs. By default, the scene visualization is essentially a birds-eye-view of the environment that shows all of the objects in all dimensions (Figure \ref{fig:default_view}). \textit{Objects} are visualized as a simple yet easily recognizable icon, and they are placed in different areas of the cell depending on the vertical dimension that it is in. \textit{Furniture} is rendered as a colored background. In this view, \textit{object} states are not shown, but \textit{furniture} states are. 

% Still, it is possible to view the states of all objects in the cell directly in front of the agent as this includes all of the objects that the agent can interact with at that point. The user is able to open a 'Closeup' of the cell on the right of the grid, which displays 4 squares for the three dimensions and furniture in the cell. For each square, the icon and states are rendered. 

% \begin{figure}[ht]
%     \centering    \includegraphics[width=1\textwidth]{default_view.png}
%     \caption{Default view of the grid -- showing all objects as icons and all furniture as a colored background. All furniture states are shown in the grid with a green edge, while object states are only visualized for the cell directly in front of the agent by a red or green box.}
%     \label{fig:default_view}
% \end{figure}

% \subsection{Scene Visualization: Furniture Only and Single Dimension}
% The dimension view is used to visualize a single vertical dimension (top, middle, or bottom), and it shows all objects, furniture, and states in the specified dimension. Similar to the default view, objects are rendered as icons while furniture is a colored background. The key difference is that the object icon takes up the full cell, and the object states are visualized in addition to the furniture states.

% In the furniture-only view, the \textit{furniture} icons are displayed, and no \textit{objects} or object states are shown. 

% \begin{figure}[ht]
%     \centering    \includegraphics[width=1\textwidth]{other_views.png}
%     \caption{Other views of the grid -- (left) Furniture only view only shows furniture and furniture state. (right) Single dimension view of the bottom dimension, which shows all furniture and objects in the bottom dimension with their states. Comparing with the default view (Figure \ref{fig:default_view}), we see that the 'apple' from the closeup corresponds to the cell in front of the agent in the single dimension view}
%     \label{fig:enter-label}
% \end{figure}

% % \begin{table}[h]
% %     \centering
% %     \begin{tabular}{|c|c|c|c|c|c|}
% %     \hline
% %        View Type & Objs Shown & Object Icon & Object State & Furniture Icon & Furniture State \\
% %        \hline
% %         Default & all & \checkmark & & & \checkmark \\
% %         \hline
% %         Single Dimension & 1 & \checkmark & \checkmark & & \checkmark \\
% %         \hline         
% %         Furniture Only & 0 & & & \checkmark & \checkmark \\
% %         \hline      
% %         \end{tabular}
% %     \caption{Summary of the Different Views and Features}
% %     \label{tab:my_label}
% % \end{table}

% \subsection{General Usage: Defining Tasks and Initializing Scenes}

% \label{sec:usage}

% Each task is defined by a set of objects, initial conditions, and goal conditions. 

% When a scene is initialized, it contains all objects required by the task, and the objects are placed to satisfy all of the initial conditions. This is done randomly by default, but it is also possible to procedurally generate scenes as described in the previous section. The goal of the agent is to navigate and manipulate the scene in a way such that all of the goal conditions are eventually satisfied. 

% We provide a standardized set of 20 tasks with conditions in the BEHAVIOR Domain Definition Language (BDDL), which we will detail more in section 3. However, it is also easy to create new tasks, objects, and actions using the classes and modules that we provide.  

% \subsection{General Usage: Control Modes}
% We support two modes: agent control and manual control. In the agent control mode, the agent is controlled by an algorithm, and this is useful for training different RL and planning agents. In manual control, a user can manually navigate and interact with the environment using keyboard controls. This is useful for creating human demonstrations.
